Bound states of WIMP dark matter in Higgs-portal models. Part I. Cross-sections and transition rates

We investigate the role of the Higgs \emph{doublet} in the thermal decoupling of multi-TeV dark matter coupled to the Weak interactions of the Standard Model and the Higgs. The Higgs doublet can mediate a long-range force that affects the annihilation processes and binds dark matter into bound states. More importantly, the emission of a Higgs doublet by a pair of dark matter particles can give rise to extremely rapid monopole bound-state formation processes and bound-to-bound transitions. We compute these effects in the unbroken electroweak phase. To this end, we consider the simplest renormalisable fermionic model, consisting of a singlet and a doublet under $SU_{L}(2)$ that are stabilised by a $\mathbb{Z}_2$ symmetry, in the regime where the two multiplets coannihilate. In a companion paper, we use the results to show that the formation of metastable bound states via Higgs-doublet emission and their decay decrease the relic density very significantly.

==> FiguresAndTables/Table_Annihilation.tex <==
\renewcommand*{\arraystretch}{1}
\begin{align*}
\begin{array}{|c|c|c|c|c|c|c|}
\hline 
 \text{Channel}
&\UY
&\SUL
&\text{Spin}
&\text{dof}
&(\sigma_{_0} \vrel) / (\pi m^{-2})
&\text{Sommerfeld factor}
\\ \hline \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SS \to HH^\dagger
&0
&\mathbb{1}
&0,1
&4
&0
&-
\\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{$D\bar{D} \to HH^\dagger$}
&\multirow{4}{*}{0}
&\multirow{2}{*}{$\mathbb{1}$}
&0
&1
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&3
& (\alpha_1+2\aH)^2/12
& S_0 \[(\zeta_1+3\zeta_2)/4\]
\\ \cline{3-7}
%%%
&%%
&\multirow{2}{*}{$\mathbb{3}$}
&0
&3
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&9
& (\alpha_2+2\aH)^2/12
& S_0 \[(\zeta_1-\zeta_2)/4\]
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{$D\bar{D} \to WW$}
&\multirow{4}{*}{0}
&\multirow{2}{*}{$\mathbb{1}$}
&0
&1
&3\alpha_2^2/2
&\dfrac{\aA S_0(\zetaA) + \aR S_0(-\zetaR)}{\aA+\aR}
%\Sigma~~\text{[cf.~\cref{eq:GaugeSingletSpin0_Sommerfeld}]}
\\ \cline{4-7}
%%%
&%%
&%%
&1
&3
&0
&-
\\ \cline{3-7}
%%%
&%%
&\multirow{2}{*}{$\mathbb{3}$}
&0
&3
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&9
& \alpha_2^2/12
& S_0 \[(\zeta_1-\zeta_2)/4\]
\\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{$D\bar{D} \to BB$}
&\multirow{3}{*}{0}
&\multirow{2}{*}{$\mathbb{1}$}
&0
&1
& \alpha_1^2/2
&\dfrac{\aA S_0(\zetaA) + \aR S_0(-\zetaR)}{\aA+\aR}
\\ \cline{4-7}
%%%
&%%
&%%
&1
&3
&0
&-
\\ \cline{3-7}
%%%
&%%
&\mathbb{3}
&0,1
&12
&0
&-
\\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{$D\bar{D} \to WB$}
&\multirow{3}{*}{0}
&\mathbb{1}
&0,1
&4
&0
&-
\\ \cline{3-7}
%%%
&%%
&\multirow{2}{*}{$\mathbb{3}$}
&0
&3
&\alpha_1\alpha_2
& S_0 \[ (\zeta_1-\zeta_2)/4 \]
\\ \cline{4-7}
%%%
&%%
&%%
&1
&9
&0
&-
\\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{$D\bar{D} \to F_{\mathsmaller{L}} \bar{F}_{\mathsmaller{L}}$}
&\multirow{4}{*}{0}
&\multirow{2}{*}{$\mathbb{1}$}
&0
&1
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&3
&\parbox{15ex}{\centering 
$2 Y_{\mathsmaller{L}}^2 \alpha_1^2/3,$ \\ 
$\sum Y_{\mathsmaller{L}}^2 = 1$}
&S_0 \[ (\zeta_1+3\zeta_2)/4 \]
\\ \cline{3-7}
%%%
&%%
&\multirow{2}{*}{$\mathbb{3}$}
&0
&3
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&9
&\parbox{15ex}{\centering $N_\mathsmaller{L} \times \alpha_2^2/6$ \\ $N_\mathsmaller{L} = 12$}
& S_0 \[ (\zeta_1-\zeta_2)/4 \]
\\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{$D\bar{D} \to f_{\mathsmaller{R}} \bar{f}_{\mathsmaller{R}}$}
&\multirow{3}{*}{0}
&\multirow{2}{*}{$\mathbb{1}$}
&0
&1
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&3
&\parbox{15ex}{\centering 
$Y_{\mathsmaller{R}}^2 \alpha_1^2/3,$ \\ 
$\sum Y_{\mathsmaller{R}}^2 = 8$}
& S_0 \[ (\zeta_1+3\zeta_2)/4 \]
\\ \cline{3-7}
%%%
&%%
&\mathbb{3}
&0,1
&12
&0
&-
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{$DD \to H H$}
&\multirow{3}{*}{1}
&\multirow{2}{*}{$\mathbb{1}$}
&0
&1
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&3
&4\aH^2/3 
&S_0 \[(-\zeta_1+3\zeta_2)/4\]
\\ \cline{3-7}
%%%
&%%
&\mathbb{3}
&0,1
&12
&0
&-
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{2}{*}{$DS \to W H$}
&\multirow{2}{*}{1/2}
&\multirow{2}{*}{$\mathbb{2}$}
&0
&2
&0
&-
\\ \cline{4-7}
%%%
&%%
&%%
&1
&6
&\alpha_2 \aH/2
&S_0(-\zetaH)
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{2}{*}{$DS \to B H$}
&\multirow{2}{*}{1/2}
&\multirow{2}{*}{$\mathbb{2}$}
&0
&2
&0
&-%S_0(+\zetaH)
\\ \cline{4-7}
%%%
&%%
&%%
&1
&6
&\alpha_1 \aH/6
&S_0(-\zetaH)
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DS \to f_{\mathsmaller{R}} \bar{F}_{\mathsmaller{L}}
&1/2
&\mathbb{2}
&0,1
&8
&0
&-
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DS \to F_{\mathsmaller{L}} \bar{f}_{\mathsmaller{R}}
&1/2
&\mathbb{2}
&0,1
&8
&0
&-
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{array}
\end{align*}
